DualCoOp++: Fast and Effective Adaptation to Multi-Label Recognition with Limited Annotations

Multi-label image recognition in the low-label regime is a task of great challenge and practical significance. Previous works have focused on learning the alignment between textual and visual spaces to compensate for limited image labels, yet may suffer from reduced accuracy due to the scarcity of high-quality multi-label annotations. In this research, we leverage the powerful alignment between textual and visual features pretrained with millions of auxiliary image-text pairs. We introduce an efficient and effective framework called Evidence-guided Dual Context Optimization (DualCoOp++), which serves as a unified approach for addressing partial-label and zero-shot multi-label recognition. In DualCoOp++ we separately encode evidential, positive, and negative contexts for target classes as parametric components of the linguistic input (i.e., prompts). The evidential context aims to discover all the related visual content for the target class, and serves as guidance to aggregate positive and negative contexts from the spatial domain of the image, enabling better distinguishment between similar categories. Additionally, we introduce a Winner-Take-All module that promotes inter-class interaction during training, while avoiding the need for extra parameters and costs. As DualCoOp++ imposes minimal additional learnable overhead on the pretrained vision-language framework, it enables rapid adaptation to multi-label recognition tasks with limited annotations and even unseen classes. Experiments on standard multi-label recognition benchmarks across two challenging low-label settings demonstrate the superior performance of our approach compared to state-of-the-art methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/different_N_partial_label.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Performance of different $N-$s with 10\% labels on MS-COCO} }~\label{table:different_n_-_plmlc}
    % \vspace{-30pt}
        \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{c c c c c c c c }
            \Xhline{3\arrayrulewidth} 
            (N_+, N_-) &  CP & CR & CF1 & OP & OR & OF1 & mAP \\
            \Xhline{3\arrayrulewidth} 
            (16, 2) & 67.1 & 77.9& 71.8 & 69.8 & 82.2 &	75.5 & 78.7 \\
            (16, 4) & 67.7 & 77.6 & 72.1 & 70.3 & 81.8& 75.6 & 78.7 \\
            (16, 8) & 68.4 & 77.8 & 72.6 & 70.9 &  81.8 & 76.0 & 78.9 \\
            (16, 16) & 69.1 & 77.5 & 72.6 &	71.4 & 81.6 & 76.2 & 78.7 \\
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}

==> tables/different_N_zsl.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Zero-Shot performance of different $N-$s on MS-COCO} }~\label{table:different_n_-_zsmlc}
    % \vspace{-30pt}
        \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{c c c c c c c }
            \Xhline{3\arrayrulewidth} 
            (N_+, N_-) &  ZS-P & ZS-R & ZS-F1 & GZS-P & GZS-R & GZS-F1  \\
            \Xhline{3\arrayrulewidth} 
            (32, 2) & 31.2 & 77.4 &	44.4 & 55.1	& 64.3 & 59.3 \\
            (32, 4) & 33.1 & 82.1 &	47.1 & 57.1 & 66.6 & 61.5 \\
            (32, 8) & 34.0 &  84.4 & 48.4 &  57.6 & 67.2 &	62.0 \\
            (32, 16) & 34.8 & 86.6 & 49.7 &  57.5 &	67.1 & 61.9 \\
            (32, 32) & 35.8 & 88.9 & 51.0 &	57.4 & 67.0 & 61.9 \\ 
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}

==> tables/different_attn.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Comparison among different aggregation functions on MS-COCO using partial labels}}~\label{table:different_attn}
    % \vspace{-30pt}
        \resizebox{0.6\linewidth}{!}{
        \begin{tabular}{c c c c c c  }
            \Xhline{3\arrayrulewidth} 
            Aggregation &  $10\%$  & $30\%$ & $50\%$ & $70\%$ & $90\%$ \\
            \Xhline{3\arrayrulewidth} 
            Average & 67.6 & 67.6 & 71.9 & 72.5 & 72.8\\
            Max & 66.7 & 72.8 & 75.5 & 75.8 & 76.5\\
            Softmax (\ours) & \textbf{78.4} & \textbf{81.0} & \textbf{82.0} & \textbf{82.5}  & \textbf{82.8}  \\
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}

==> tables/full_performance_big_earth.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Performance of MLR with partial labels on BigEartn}}~\label{table:bigearth_full}
    % \vspace{-30pt}
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{c c c c c c c c }
            \Xhline{3\arrayrulewidth} 
            Amount of Labels & CP & CR & CF1& OP & OR & OF1 & mAP \\
            \Xhline{3\arrayrulewidth} 
            10\% & 76.9 & 84.3 &  78.8 &  71.9 &  85.9 &  78.3 & 88.2 \\
            20\% &  81.6 & 94.2 & 86.9 &  73.4 & 93.1 & 82.1 & 92.9 \\
            30\% & 83.7 & 93.1 & 87.4 &	75.7 & 92.5 & 83.3 & 93.1 \\
            40\% &  82.7 &	93.9 &	87.2 &	75.8 &	92.0 &	83.1 &	93.5 \\
            50\% &  81.3 & 93.2 & 85.9 & 74.4 &	90.4 &	81.6 &	93.7 \\
            60\% &  86.2 &	92.3 &	88.9 &	80.2 &	91.1 &	85.3 & 94.3\\
            70\% &  86.0 &	92.8 &	88.8 &	79.4 &	91.7 &	85.1 & 94.2 \\
            80\% &  85.1 &	94.8 &	89.2 & 77.9 & 93.2 & 84.9 &	94.1 \\
            90\% &  83.9 & 94.4 & 88.2 & 77.2 &  93.4 & 84.5 & 94.7 \\
            100\% (No Finetune) & 85.8 & 95.5 &	90.0 & 78.7 & 93.8 & 85.6 & 95.2 \\
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}

==> tables/full_performance_mscoco.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Performance of MLR with partial labels on MS-COCO}}~\label{table:ms_coco_full}
    % \vspace{-30pt}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c c c c c c c c }
            \Xhline{3\arrayrulewidth} 
            Amount of Labels & CP & CR & CF1& OP & OR & OF1 & mAP \\
            \Xhline{3\arrayrulewidth} 
            10\% &  69.1 &	77.5 &	72.6 &	71.4 &	81.6 & 	76.2 &	78.7 \\
            20\% & 70.1 & 79.4 & 74.2 &	72.1 & 83.0 & 77.2 & 80.9 \\
            30\% & 71.2. & 	80.1 &	75.1. &	72.9. &	83.5 &	77.8 &	81.7 \\
            40\% & 71.3 & 80.2 & 75.2 & 73.2  & 83.8 &	78.1 &	82.0 \\
            50\% & 72.1	& 80.4 & 75.8 & 73.7 & 83.9 &	78.5. &	82.5\\
            60\% & 72.4 & 80.6 & 76.0 & 73.9 &	84.0 &	78.6 &	82.7\\
            70\% & 72.5 & 80.5 & 76.1 &	74.1 &	83.9 & 78.7 & 82.8\\
            80\% & 72.9 & 80.7 & 76.3 &	74.3 &	84.1 & 78.9 & 83.0 \\
            90\% & 72.9 & 80.7 &  76.4	& 74.5 & 84.1 &	79.0	&83.1 \\
            100\% (No Finetune) & 73.2 & 80.8 & 76.6 & 74.6 & 84.2 & 79.1 &	83.2 \\
            100\% (Finetune Aggre. Func.) & 75.7 & 80.4 & 77.8 & 77.1 & 	83.7 & 	80.3 & 84.2 \\
            100\% (Finetune Img. Enc.) &  92.5 &  68.0 & 77.3 &	93.5  & 70.8	 & 80.6 &	85.3 \\
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}

==> tables/full_performance_voc.tex <==
\begin{table}
    \begin{center}
     \caption{\small \textbf{Performance of MLR with partial labels on VOC2007}}~\label{table:voc_full}
    % \vspace{-30pt}
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{c c c c c c c c }
            \Xhline{3\arrayrulewidth} 
            Amount of Labels & CP & CR & CF1& OP & OR & OF1 & mAP \\
            \Xhline{3\arrayrulewidth} 
            10\% &  69.6 &	91.3 &	78.0 & 	72.4 &	92.4 &	81.2 &	90.3  \\
            20\% & 74.2 & 	92.6 &	81.7 &	76.2 &	93.6 &	84.0 & 92.2  \\
            30\% & 74.9 & 92.8 & 82.3 &	78.6 &	93.3 &	85.3 &	92.8 \\
            40\% & 78.4 & 92.5 & 84.5 & 80.8 & 93.3 & 86.6 & 93.3  \\
            50\% & 80.6 & 93.4 & 86.3 &	82.4 &	94.0 &	87.8 &	93.6 \\
            60\% & 80.1 & 93.7 & 86.0 &	81.4 &	94.4 &	87.4 &	93.9 \\
            70\% & 80.9 & 93.4 & 86.5 &	82.7 & 94.0 & 88.0 & 94.0 \\
            80\% & 80.8 & 93.8 & 86.5 &  82.9 & 94.2 & 88.2 & 94.1  \\
            90\% & 80.5	& 93.9 &	86.3 &	82.4 &	94.4 &	88.0 &	94.2 \\
            100\% (No Finetune) &  81.2 & 94.1 & 86.8 & 83.2 & 94.5 & 88.5 & 	94.4\\
             \Xhline{3\arrayrulewidth} 
        \end{tabular}
        } 
    \end{center}
% \vspace{-35pt}
\end{table}
